RAS: Retrieval-And-Structuring for Knowledge-Intensive LLM Generation

Large language models (LLMs) have achieved impressive performance on knowledge-intensive tasks, yet they often struggle with multi-step reasoning due to the unstructured nature of retrieved context. While retrieval-augmented generation (RAG) methods provide external information, the lack of explicit organization among retrieved passages limits their effectiveness, leading to brittle reasoning pathways. Recent interpretability studies highlighting the importance of structured intermediate reasoning further align with this perspective. We propose Retrieval-And-Structuring (RAS), a framework that dynamically constructs question-specific knowledge graphs through iterative retrieval and structured knowledge building. RAS interleaves targeted retrieval planning with incremental graph construction, enabling models to assemble and reason over evolving knowledge structures tailored to each query. On seven knowledge-intensive benchmarks, RAS consistently outperforms strong baselines, achieving up to 8.7\% and 7.0\% gains with proprietary and open-source LLMs, respectively. Our results demonstrate that dynamic, question-specific knowledge structuring offers a robust path to improving reasoning accuracy and robustness in language model generation.

==> figures/classifier_shifter_train.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/dbpedia_metrics.pdf}
        \vspace{-2em}
        \caption{\textbf{Multilabel Document Classifier Training}. It shows the training metrics for the multilabel document classifier, including validation precision, recall, and F1 score.}
        \label{fig:classifier_train}
    \end{subfigure}
    \vspace{2em}  % Space between subfigures
    
    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/shifter_all_metrics_.pdf}
        \vspace{-2em}
        \caption{\textbf{Distribution Shifter Training}. It displays various distance metrics used to evaluate the quality of distribution alignment.}
        \label{fig:shifter_train}
    \end{subfigure}
    \vspace{2em}

    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/t2t_metrics.pdf}
        \vspace{-2em}
        \caption{\textbf{Text-to-Triple Model Training}. It shows the validation rouge scores to evaluate the extracted triple list.}
        \label{fig:t2t_train}
    \end{subfigure}
    \label{fig:training_reports}
\end{figure*}

==> figures/efficiency_study.tex <==
\begin{wrapfigure}
\centering
\includegraphics[width=\linewidth]{figures/efficiency_study_.pdf}
\vspace{-2em}
\caption{Efficiency study of RAS conducted on our machine. For RAS, we set \#iteration=2 and use closed-source LLM for illustration. The result is averaged over 100 TriviaQA samples tested. $K$=250,000 and $k$=5 are set in this case. The Wiki 2018 dump ($\sim$ 32M documents) is used and loaded on CPU for this analysis. }
\label{fig:efficiency}
% \vspace{-1em}
\end{wrapfigure}

==> figures/graph_abundance.tex <==
\begin{figure}[t]
% \vspace{-2em}
\centering
\includegraphics[width=\linewidth]{figures/graph_size_vs_performance.pdf}
\vspace{-1.5em}
\caption{Impact of Graph Information Abundance on Model Performance. For each sample, we randomly shuffle its associated triples five times and take different ratios (10\%, 30\%, 50\%, 70\%, 100\%) of the shuffled data. The performance scores shown are averaged across these five shuffling runs.}
\label{fig:graph_ab}
\vspace{-0.5em}
\end{figure}

==> figures/overview.tex <==
\begin{figure*}[tbp]
% \vspace{-1em}
\centering
\includegraphics[width=\linewidth]{figures/ras_overview.pdf}
\vspace{-1.5em}
\caption{\small \textbf{Overview of the Retrieval-And-Structuring (RAS) framework.} RAS operates through: \textbf{(1) Planning.} Strategically determines knowledge retrieval needs and generates focused sub-queries based on the current knowledge state; \textbf{(2) Text Retrieval and Knowledge Structuring.} Retrieve text based on the sub-query and transforms the retrieved content into a graph, which is emerged to an evolving question-specific knowledge graph that expands based on reasoning needs; and \textbf{(3) Answering.} Leverage the accumulated structured knowledge to produce the final output. The framework employs parameter-efficient training to train the Graph LLM~\citep{perozzi2024let, he2024gretriever}, fine-tuning only the graph encoder, projector components, optionally with LoRA.
We provide a step-by-step running example in Figure~\ref{fig:run_example} to concretize the framework.
}
\label{fig:overview}
\end{figure*}

==> figures/overview_2.tex <==
\begin{figure*}[tbp]
\vspace{-1em}
\centering
\includegraphics[width=\linewidth]{figures/ras_overview_2.pdf}
\vspace{-1.5em}
\caption{\small \textbf{Structure-Aware Multitask Learning for the Graph LLM in RAS.}  We employ parameter-efficient training to train the Graph LLM~\citep{perozzi2024let, he2024gretriever}.}
\vspace{-0.5em}
\label{fig:overview_2}
\end{figure*}



==> old_neurips/figures/classifier_shifter_train.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/dbpedia_metrics.pdf}
        \vspace{-2em}
        \caption{\textbf{Multilabel Document Classifier Training}. It shows the training metrics for the multilabel document classifier, including validation precision, recall, and F1 score.}
        \label{fig:classifier_train}
    \end{subfigure}
    \vspace{2em}  % Space between subfigures
    
    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/shifter_all_metrics_.pdf}
        \vspace{-2em}
        \caption{\textbf{Distribution Shifter Training}. It displays various distance metrics used to evaluate the quality of distribution alignment.}
        \label{fig:shifter_train}
    \end{subfigure}
    \vspace{2em}

    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{figures/t2t_metrics.pdf}
        \vspace{-2em}
        \caption{\textbf{Text-to-Triple Model Training}. It shows the validation rouge scores to evaluate the extracted triple list.}
        \label{fig:t2t_train}
    \end{subfigure}
    \label{fig:training_reports}
\end{figure*}

==> old_neurips/figures/efficiency_study.tex <==
\begin{wrapfigure}
\centering
\includegraphics[width=\linewidth]{figures/efficiency_study_.pdf}
\vspace{-2em}
\caption{Efficiency study of RAS conducted on our machine. For RAS, we set \#iteration=2 and use closed-source LLM for illustration. The result is averaged over 100 TriviaQA samples tested. $K$=250,000 and $k$=5 are set in this case. The Wiki 2018 dump ($\sim$ 32M documents) is used and loaded on CPU for this analysis. }
\label{fig:efficiency}
% \vspace{-1em}
\end{wrapfigure}

==> old_neurips/figures/graph_abundance.tex <==
\begin{figure}[t]
% \vspace{-2em}
\centering
\includegraphics[width=\linewidth]{figures/graph_size_vs_performance.pdf}
\vspace{-1.5em}
\caption{Impact of Graph Information Abundance on Model Performance. For each sample, we randomly shuffle its associated triples five times and take different ratios (10\%, 30\%, 50\%, 70\%, 100\%) of the shuffled data. The performance scores shown are averaged across these five shuffling runs.}
\label{fig:graph_ab}
\vspace{-0.5em}
\end{figure}

==> old_neurips/figures/overview.tex <==
\begin{figure*}[tbp]
% \vspace{-1em}
\centering
\includegraphics[width=\linewidth]{figures/ras_overview.pdf}
\vspace{-1.5em}
\caption{\small \textbf{Overview of the Retrieval-And-Structuring (RAS) framework.} RAS operates through three stages: \textbf{(1) Planning} strategically determines knowledge retrieval needs and generates focused sub-queries based on the current knowledge state; \textbf{(2) Text Retrieval and Knowledge Structuring} retrieves text based on the sub-query and transforms the retrieved content into a graph, which is emerged to an evolving knowledge graph that expands based on reasoning needs; and \textbf{(3) Answering} leverages the accumulated structured knowledge to produce the final output. The framework employs parameter-efficient training to train the Graph LLM~\cite{perozzi2024let, he2024gretriever}, fine-tuning only the graph encoder, projector components, optionally with LoRA.
We provide a step-by-step running example in Figure~\ref{fig:run_example} to concretize the framework.
}
\label{fig:overview}
\end{figure*}

==> old_neurips/figures/train_size_perf.tex <==
\begin{figure*}[!t]
% \vspace{-2em}
\centering
\includegraphics[width=\linewidth]{figures/train_size_vs_performance.pdf}
\vspace{-1.5em}
\caption{\small \textbf{Impact of Training Data Volume on Model Performance.} Results for RAS$_{\text{7B}}$ (top) and RAS$_{\text{8B}}$ (bottom) illustrate how performance scales with increasing training data.}
\label{fig:train_size_perf}
% \vspace{-0.5em}
\end{figure*}

==> old_neurips/tables/ablation_study.tex <==
\begin{figure}[t]
\vspace{-1em}
\centering
\begin{minipage}[t]{0.47\textwidth}
\centering
\vspace{0pt} % Align top!
\begin{table}[H]
\small % Slightly smaller font (optional for compactness)
\setlength{\tabcolsep}{3pt} % Tighter column spacing if needed
\renewcommand{\arraystretch}{1.2} % More vertical spacing in table rows
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
& TQA & 2WQA & Pub & \multicolumn{2}{c}{ASQA} \\
& (acc) & (F1) & (acc) & (rg) & (mv) \\
\midrule
RAS$_{\text{7B}}$ & \textbf{72.7} & \textbf{42.1} & \textbf{74.7} & \textbf{37.2} & \textbf{95.2} \\
\midrule
\rowcolor{red!5}
\multicolumn{6}{c}{\textbf{\textit{Training Phase}}} \\
No GraphEncode & 70.2 & 38.4 & 66.4 & 33.1 & 85.0 \\
No LoRA & 71.5 & 37.8 & 54.8 & 32.8 & 84.8 \\
No Text-to-Triple & 70.4 & 38.2 & 71.4 & 36.2 & 73.8 \\
No Multi-Task & 68.6 & 39.2 & 65.5 & 36.7 & 88.9 \\
\midrule
\rowcolor{green!10}
\multicolumn{6}{c}{\textbf{\textit{Inference Phase}}} \\
No Retrieval & 56.9 & 27.4 & 69.0 & 31.3 & 70.6 \\
No GraphEncode & 68.8 & 38.7 & 67.3 & 36.5 & 93.6 \\
No Planning & 66.7 & 37.8 & 71.5 & 37.2 &95.2 \\
% No ThemeScope & 72.0 & n/a & 73.9 & n/a & n/a \\
\bottomrule
\end{tabular}
}
\vspace{1em}
\caption{\small \textbf{Ablations in Training and Inference (with RAS$_{7\text{B}}$).} \underline{\textbf{Training}}: ``No GraphEncode'' removes the graph encoder during training, using only LoRA-based LLM fine-tuning. ``No LoRA'' uses graph token optimization without low-rank adaptation. ``No Text-to-Triple'' keeps the original retrieved texts instead of converting them into triples. ``No Multi-Task'' trains two models separately handling planning and answering. \underline{\textbf{Inference}}: ``No Retrieval'' tests direct query answering without any context. ``No GraphEncode'' removes graph encoding and projection during inference, using only textual context. ``No Planning'' removes the planning module and runs single-pass retrieval-structuring-answering pipeline. }
\label{tb:ablation}
\end{table}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
\centering
\vspace{1em} % Align top!
\includegraphics[width=\linewidth]{figures/role_swapping_ras.pdf}
\vspace{-1em} 
\caption{\small
\textbf{Role-Swapping Study.} We alternate Sonnet-3.5 and RAS$_\text{7B}$ on the planning and answering tasks, and evaluate the overall performance.
}


\label{fig:role_swap}
\vspace{0.8em} % Little breathing room between figures
\includegraphics[width=\linewidth]{figures/graph_size_vs_performance.pdf}
\vspace{-1.2em}
\caption{\small \textbf{Impact of Graph Information Abundance.} For each sample, we randomly shuffle its associated triples five times and take different ratios (10\%–100\%) of the shuffled data. The performance scores are averaged across these five shuffling runs.}
\vspace{-1em}
\label{fig:graph_ab}
\end{minipage}
\end{figure}


==> old_neurips/tables/hotpot_stat.tex <==
% Requires packages: booktabs, multirow
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llll}
\toprule
& & Planning Data &Answering Data \\
\midrule
\# Queries & &129,902  & 78,164 (w/ 3,897 ASQA \& 2,147 Arc-Easy)\\
\# Input Tokens &(Mean, Median, Max)  & (338, 301, 1,910)  & (475, 466, 2,214) \\
\# Output Tokens &(Mean, Median, Max) & (13, 12, 62)  & (13, 4, 2,332) \\
\# Subqueries  & (Min, Mean, Max) &(0, 0.8, 5)  &(0, 1.2, 6) \\
\# \texttt{[SUFFICIENT]}    &&45,722 &--\\
\# \texttt{[SUBQ]} &&71,676   &--\\
\# \texttt{[NO\_RETRIEVAL]} &&12,504 &--\\
\# \texttt{[SUBQ]} Tokens & (Min, Mean, Max) &(6, 18.3, 62)  &--\\
\# Nodes & (Mean, Median, Max) & (11.6, 11, 56)   & (11.7, 11, 84) \\
\# Edges & (Mean, Median, Max) & (21.2, 20, 116)  & (21.3, 20, 160) \\

\bottomrule

\end{tabular}
}
\vspace{1em}
\caption{Statistics of our constructed HotpotQA-SUBQ dataset.}

\label{tb:hotpot_stat}
\vspace{-1em}
\end{table}

==> old_neurips/tables/hyper_study.tex <==
\begin{table*}[!h]
\centering
\captionof{table}{Hyper-parameter study. We \textbf{highlight} the setting used in experiments.}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ll}
\toprule
\textbf{Hyper-parameter} & \textbf{Studied Values} \\
\midrule
% \textbf{Theme Classifier} \\
% Encoder learning rate & \{1e-6, 1e-5, \textbf{2e-5}, 1e-4, 2e-4\}  \\
% Classifier learning rate & \{1e-6, 1e-5, 2e-5, 1e-4, \textbf{2e-4}, 5e-4, 1e-3\}  \\
% Batch size & \{4, 8, \textbf{16}, 32, 64\}\\
% Hidden layers & \{\textbf{1}, 2, 3\}  \\
% Hidden dim & \{256, \textbf{512}, 1024\} \\
% Dropout rate & \{\textbf{0.1}, 0.2, 0.3\} \\

% \midrule
% \textbf{Distribution Shifter} \\
% Batch size & \{4, 8, 16, \textbf{32}, 64\} \\
% Learning rate & \{0.0001, 0.0005, \textbf{0.001}, 0.005\} \\
% Hidden layers & \{[256], [512], [\textbf{512, 256}], [1024, 512, 256]\} \\
% Dropout rate & \{0.1, 0.15, \textbf{0.2}, 0.25, 0.3\} \\
% Optimizer & \{\textbf{Adam}, SGD, RMSprop, AdamW\} \\
% Loss function & \{\textbf{KLDiv}, JSD, MSE, Wasserstein, CrossEntropy\} \\

% \midrule
\textbf{Text-to-Triples Model} \\
Batch size & \{2, 4, \textbf{8}, 16, 32\} \\
Learning rate & \{1e-5, 2e-5, \textbf{5e-5}, 1e-4, 2e-4\} \\


\midrule
\textbf{GraphLLM (Action Planner \& Answerer)} \\
\hdashline
\multicolumn{2}{l}{\textit{GNN Setting (for Graph Token)}} \\
GNN architecture & \{GCN, GAT, \textbf{Graph Transformer}\} \\
Hidden dimension & \{512, 768, \textbf{1024}, 2048\} \\
Number of layers & \{2, \textbf{3}, 4, 5\} \\
Number of heads & \{4, 6, \textbf{8}, 12\} \\
Dropout rate & \{0.05, \textbf{0.1}, 0.2, 0.3\} \\
Projector intermediate dimension & \{1024, \textbf{2048}, 4096\} \\
Projector output dimension & \textbf{4096} \\
\hdashline
\textit{LoRA Setting} \\
LoRA rank (r) & \{4, \textbf{8}, 16, 32\} \\
LoRA alpha & \{8, \textbf{16}, 32\} \\
LoRA dropout & \{0.01, \textbf{0.05}, 0.1, 0.15\} \\
\hdashline
\multicolumn{2}{l}{\textit{General Setting}} \\
Learning rate & \{1e-6, 2e-6, \textbf{5e-5}, 1e-4\} \\
Batch size (training) & \{\textbf{2}, 4, 8, 16, 32\} \\
Batch size (inference) & \textbf{1} \\
Weight decay & \{0.001, \textbf{0.01}, 0.05, 0.1\} \\
Gradient accumulation steps & \{\textbf{2}, 4, 8, 16\} \\
Gradient clipping & \{0.1, 0.3, \textbf{0.5}, 1.0\} \\
Warmup ratio & \{0.05, 0.1, \textbf{0.15}, 0.2\} \\
Max text length & \textbf{2500} \\
Max new tokens & Task-specific (see Appendix \ref{apsub:open_setting}) \\
\midrule
\textbf{Others} \\
% Theme scoping top-$K$ & \{100,000, \textbf{250,000}, 500,000 \}\\
Dense retrieval top-$k$ & \textbf{5} \\

\bottomrule
\end{tabular}
}
\label{tb:hyperparams}
\end{table*}

==> old_neurips/tables/main_results.tex <==
% Requires packages: booktabs, multirow
\begin{table*}[t]
\vspace{-1em}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
&  \multicolumn{3}{c}{Short-form} & \multicolumn{2}{c}{Closed-set} & \multicolumn{4}{c}{Long-form Generation} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-10}
Model   & TQA &2WQA & PopQA & Pub & ARC  & \multicolumn{2}{c}{ASQA} &\multicolumn{2}{c}{ELI5} \\
&  (acc) &(F1) & (acc) & (acc) & (acc)  & (rouge)  & (mauve) & (rouge)  & (mauve)\\
\midrule
\rowcolor{blue!10}
\multicolumn{10}{c}{\small {Baselines w/o Retrieval}} \\
Llama2$_{7\text{B}}$ & 30.5 & 18.9 & 14.7 & 34.2 & 21.8   & 15.3 &19.0 &18.3 &32.4 \\
Alpaca$_{7\text{B}}$ & 54.5 & -- & 23.6 & 49.8 & 45.0   & 29.4 & 61.7 & -- & -- \\
Llama2$_{13\text{B}}$ & 38.5 & 20.2 & 14.7 & 29.4 & 29.4   & 12.4 &16.0 &18.2 & 41.4 \\
Alpaca$_{13\text{B}}$ & 61.3 & -- & 24.4 & 55.5 & 54.9   & 32.0 & 70.6 & -- & -- \\
Llama3$_{8\text{B}}$ &56.1 &21.2 &26.7 &33.2 &42.2 &17.6 &25.0 &18.2 &39.7 \\
ChatGPT$_{\sim 175\text{B}}$ & 74.3 &24.8 & 29.3 & 70.1 & 75.3   & 36.2 & 68.8 &\textcolor{secondclose}{22.8} &32.6\\
Sonnet-3.5$_{\sim 175\text{B}}$ & \textcolor{firstclose}{\underline{78.4}} & 40.0 & 30.2  & \textcolor{firstclose}{\underline{83.7}} &88.5  &37.0 &39.1 &21.8 &26.5  \\

% \midrule
\rowcolor{blue!10}
\multicolumn{10}{c}{\small {Baselines w/ Retrieval (\#docs=5 by default)}} \\
Llama2$_{7\text{B}}$ & 42.5 &21.0 & 38.2 & 30.0 & 48.0   & 22.1 & 32.0 &18.6 &35.3 \\
Alpaca$_{7\text{B}}$ & 64.1 & -- & 46.7 & 40.2 & 48.0   & 33.3 &57.9 &-- &--\\
% Llama2-FT$_{7\text{B}}$ & & 57.3 & -- & 48.7 & 64.3 & 65.8   & 35.8 &51.2 &-- &--\\
Llama2$_{13\text{B}}$ & 47.0 & 31.2 & 45.7 & 30.2 & 26.0   & 20.5 &24.7 & 18.6 &42.3\\
Llama3$_{8\text{B}}$ &60.4 &33.4 &48.6 &36.5 &40.1 &23.9 &52.1 &18.8 &40.7\\
Alpaca$_{13\text{B}}$ & 66.9 & -- & 46.1  & 51.1 & 57.6   & 36.7 &56.6 &-- &-- \\
% Llama2-c$_{13\text{B}}$ & & 59.8 & -- & 51.8 & 52.1 & 37.9   & 34.8 &43.8 &-- &-- \\
{RECOMP$_{7\text{B}}$ \cite{xu2023recomp}}  &-- &32.4 &-- &-- &-- &36.5 &76.0 &-- &-- \\
ChatGPT & 65.7 &32.8  & 50.8 & 54.7 & 75.3   & \textcolor{firstclose}{\underline{39.9}} &\textcolor{firstclose}{\underline{79.7}} &20.6 &\textcolor{firstclose}{\underline{57.2}} \\
Sonnet-3.5$_{\#\text{docs}=1}$   &69.1 &41.9 &51.5 &49.1 &88.6  &-- &-- &-- &--\\
Sonnet-3.5$_{\#\text{docs}=5}$   &72.5 &\textcolor{secondclose}{53.7} &\textcolor{secondclose}{57.3} &53.9 &87.1   &38.8 & 61.6 &20.2 &32.3 \\
{SuRe$_{7\text{B}}$ \cite{kim2024sure}} &51.2 &20.6 &39.0  & 36.2 &52.7  &35.8 &76.2 &16.1 &26.6\\
{SuRe$_{\text{GPT}}$} &72.3 &38.1 &53.6  & 57.2 &79.6  &36.0 &74.2 &19.2 &51.6\\
{SuRe$_{\text{Sonnet-3.5}}$} &76.8 &37.6 &41.2  &62.8  &\textcolor{secondclose}{91.6}  &30.2 &69.9 &15.4 &27.2\\
% \midrule
\rowcolor{blue!10}
\multicolumn{10}{c}{\small {Baselines w/ Self-Reflective Retrieval}} \\
{Self-RAG$_{7\text{B}}$ \cite{asai2023self}} & \textcolor{secondopen}{66.4} & 25.1 & 54.9 & 72.4 & \textcolor{secondopen}{67.3}   & 35.7 &74.3 &17.9 &35.6 \\
{Self-RAG$_{13\text{B}}$} & 69.3 & -- & 55.8 & 74.5 & 73.1   & 37.0 &71.6 &-- &-- \\
{RPG$_{7\text{B}}$ \cite{lyu2024retrieve}} &65.1 &33.6 & \textcolor{secondopen}{56.0} &\textcolor{secondopen}{73.4} & 65.4  &\textcolor{secondopen}{\underline{37.6}} &\textcolor{firstopen}{84.4} &\textcolor{secondopen}{19.1} & \textcolor{firstopen}{{46.4}} \\
Search-R1$_{7\text{B}}$~\cite{jin2025search} &63.8 &\textcolor{secondopen}{35.2}  &45.7 &69.4 &64.4 &35.2 &72.3 &18.4 &37.1\\
% \midrule
\rowcolor{yellow!10}
\multicolumn{10}{c}{\small \textbf{{Retrieval-And-Structuring (RAS)}}} \\% $\mathcal{M}_{Plan}$  & $\mathcal{M}_{Ans}$ \\
RAS$_{\text{Sonnet-3.5}}$ &\textcolor{secondclose}{77.6} & \textcolor{firstclose}{\underline{57.7}} &\textcolor{firstclose}{\underline{62.3}} & \textcolor{secondclose}{71.3} &\textcolor{firstclose}{\underline{93.9}}   &\textcolor{secondclose}{39.1} & \textcolor{secondclose}{70.5}  &\textcolor{firstclose}{\underline{23.3}}  &\textcolor{secondclose}{37.7}   \\
% RAS$_{\text{Sonnet-3.5}}$ & RAS$_{7\text{B}}$ &73.8 &43.4 &61.3 &75.5 & 62.4 & 37.2 &95.2  &19.7 & 47.8\\
% RAS$_{7\text{B}}$ & RAS$_{\text{Sonnet-3.5}}$ &78.7  &54.7 &58.8  &70.8 &91.2 &39.1 &70.5  & 23.3 &37.7\\
RAS$_{8\text{B}}$  &73.8 & 44.2 &57.7 &77.6 & 71.4 &37.6 &96.2 &20.1 &54.4 \\
RAS$_{7\text{B}}$  &\textcolor{firstopen}{\underline{72.7}} &\textcolor{firstopen}{\underline{42.1}} &\textcolor{firstopen}{\underline{58.3}}  &\textcolor{secondopen}{\underline{74.7}} &\textcolor{firstopen}{\underline{68.5}} &\textcolor{firstopen}{37.2} &\textcolor{secondopen}{\underline{95.2}} & \textcolor{firstopen}{\underline{19.7}} &\textcolor{secondopen}{\underline{47.8}} \\
% [2pt]
% \hdashline[2pt/2pt] \\ [-9pt]
\bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{\small \textbf{Performance Comparison.} We highlight the \textcolor{firstclose}{top-2 closed-source models} and \textcolor{firstopen}{top-2 open-source 7B models}, underlining the \underline{best closed-/open-source (7B) model} for each dataset. Note: RAS is designed for general open-domain question answering and is not tailored for Knowledge Graph Question Answering (KGQA) tasks~\cite{perevalov-etal-2022-knowledge}; therefore, we do not compare it to KGQA-focused methods~\cite{sun2023think,luo2023reasoning,ma2024think}.}
\label{tb:main_results}
% \vspace{-1em}
\end{table*}

==> tables/main_results.tex <==
% Requires packages: booktabs, multirow
\begin{table*}[t]
\vspace{-1em}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
&  \multicolumn{3}{c}{Short-form} & \multicolumn{2}{c}{Closed-set} & \multicolumn{4}{c}{Long-form Generation} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-10}
Model   & TQA &2WQA & PopQA & Pub & ARC  & \multicolumn{2}{c}{ASQA} &\multicolumn{2}{c}{ELI5} \\
&  (acc) &(F1) & (acc) & (acc) & (acc)  & (rouge)  & (mauve) & (rouge)  & (mauve)\\
\midrule
% \rowcolor{blue!10}
% \midrule
\multicolumn{10}{l}{\textbf{w/o Retrieval}} \\
Llama2$_{7\text{B}}$ & 30.5 & 18.9 & 14.7 & 34.2 & 21.8   & 15.3 &19.0 &18.3 &32.4 \\
% Alpaca$_{7\text{B}}$ & 54.5 & -- & 23.6 & 49.8 & 45.0   & 29.4 & 61.7 & -- & -- \\
Llama2$_{13\text{B}}$ & 38.5 & 20.2 & 14.7 & 29.4 & 29.4   & 12.4 &16.0 &18.2 & 41.4 \\
% Alpaca$_{13\text{B}}$ & 61.3 & -- & 24.4 & 55.5 & 54.9   & 32.0 & 70.6 & -- & -- \\
Llama3$_{8\text{B}}$ &56.1 &21.2 &26.7 &33.2 &42.2 &17.6 &25.0 &18.2 &39.7 \\
ChatGPT$_{\sim 175\text{B}}$ & 74.3 &24.8 & 29.3 & 70.1 & 75.3   & 36.2 & 68.8 &\textcolor{secondclose}{22.8} &32.6\\
Sonnet-3.5$_{\sim 175\text{B}}$ & \textcolor{firstclose}{\underline{78.4}} & 40.0 & 30.2  & \textcolor{firstclose}{\underline{83.7}} &88.5  &37.0 &39.1 &21.8 &26.5  \\

% \midrule
% \rowcolor{blue!10}
\midrule
\multicolumn{10}{l}{\textbf{w/ Single Retrieval (\#docs=5)}} \\
Llama2$_{7\text{B}}$ & 42.5 &21.0 & 38.2 & 30.0 & 48.0   & 22.1 & 32.0 &18.6 &35.3 \\
% Alpaca$_{7\text{B}}$ & 64.1 & -- & 46.7 & 40.2 & 48.0   & 33.3 &57.9 &-- &--\\
% Llama2-FT$_{7\text{B}}$ & & 57.3 & -- & 48.7 & 64.3 & 65.8   & 35.8 &51.2 &-- &--\\
Llama2$_{13\text{B}}$ & 47.0 & 31.2 & 45.7 & 30.2 & 26.0   & 20.5 &24.7 & 18.6 &42.3\\
Llama3$_{8\text{B}}$ &60.4 &33.4 &48.6 &36.5 &40.1 &23.9 &52.1 &18.8 &40.7\\
% Alpaca$_{13\text{B}}$ & 66.9 & -- & 46.1  & 51.1 & 57.6   & 36.7 &56.6 &-- &-- \\
% Llama2-c$_{13\text{B}}$ & & 59.8 & -- & 51.8 & 52.1 & 37.9   & 34.8 &43.8 &-- &-- \\
{SuRe$_{7\text{B}}$ \citep{kim2024sure}} &51.2 &20.6 &39.0  & 36.2 &52.7  &35.8 &76.2 &16.1 &26.6\\
% ChatGPT & 65.7 &32.8  & 50.8 & 54.7 & 75.3   & \textcolor{firstclose}{\underline{39.9}} &\textcolor{firstclose}{\underline{79.7}} &20.6 &\textcolor{firstclose}{\underline{57.2}} \\
Sonnet-3.5$_{\#\text{docs}=1}$   &69.1 &41.9 &51.5 &49.1 &88.6  &n/a &n/a &n/a &n/a\\
Sonnet-3.5$_{\#\text{docs}=5}$   &72.5 &53.7 &\textcolor{secondclose}{57.3} &53.9 &87.1   &38.8 & 61.6 &20.2 &32.3 \\
{SuRe$_{\text{GPT-4o}}$} &72.3 &38.1 &53.6  & 57.2 &79.6  &36.0 &74.2 &19.2 &51.6\\
{SuRe$_{\text{Sonnet-3.5}}$} &76.8 &37.6 &41.2  &62.8  &91.6  &30.2 &69.9 &15.4 &27.2\\
% \midrule
% \rowcolor{blue!10}
\midrule
\multicolumn{10}{l}{\textbf{w/ Self-Reflective Retrieval}} \\
{Self-RAG$_{7\text{B}}$ \citep{asai2023self}} & \textcolor{secondopen}{66.4} & 25.1 & 54.9 & 72.4 & \textcolor{secondopen}{67.3}   & 35.7 &74.3 &17.9 &35.6 \\
{Self-RAG$_{13\text{B}}$} & 69.3 & 26.9 & 55.8 & 74.5 & 73.1   & 37.0 &71.6 &18.7 &38.5 \\
{RPG$_{7\text{B}}$ \citep{lyu2024retrieve}} &65.1 &33.6 & \textcolor{secondopen}{56.0} &\textcolor{secondopen}{73.4} & 65.4  &\textcolor{secondopen}{\underline{37.6}} &\textcolor{firstopen}{84.4} &\textcolor{secondopen}{19.1} & \textcolor{firstopen}{{46.4}} \\
Search-R1$_{7\text{B}}$~\citep{jin2025search} &63.8 &\textcolor{secondopen}{35.2}  &45.7 &69.4 &64.4 &35.2 &72.3 &18.4 &37.1\\
{ReAct$_{\text{7B}}$}~\citep{yao2023react} &64.0 &25.0 &42.7 &52.4 &59.0 & 22.1 & 32.0 &18.6 &35.3 \\
{IRCoT$_{\text{7B}}$}~\citep{trivedi2023interleaving} &61.5 &27.6 &44.3 &59.6 &61.6 & 22.1 & 32.0 &18.6 &35.3 \\
{ReAct$_{\text{Sonnet-3.5}}$} & 73.4 &53.7 &55.0 &62.2 &89.2 &38.8 & 61.6 &20.2 &32.3\\
{IRCoT$_{\text{Sonnet-3.5}}$} & 74.7 &\textcolor{secondclose}{54.9} &53.2 &59.4 &\textcolor{secondclose}{92.0} &38.8 & 61.6 &20.2 &32.3\\
\midrule
\multicolumn{10}{l}{\textbf{{Retrieval-And-Structuring (RAS, ours)}}} \\% $\mathcal{M}_{Plan}$  & $\mathcal{M}_{Ans}$ \\
RAS$_{\text{Sonnet-3.5}}$ &\textcolor{secondclose}{77.6} & \textcolor{firstclose}{\underline{57.7}} &\textcolor{firstclose}{\underline{62.3}} & \textcolor{secondclose}{71.3} &\textcolor{firstclose}{\underline{93.9}}   &\textcolor{secondclose}{39.1} & \textcolor{secondclose}{70.5}  &\textcolor{firstclose}{\underline{23.3}}  &\textcolor{secondclose}{37.7}   \\
% RAS$_{\text{Sonnet-3.5}}$ & RAS$_{7\text{B}}$ &73.8 &43.4 &61.3 &75.5 & 62.4 & 37.2 &95.2  &19.7 & 47.8\\
% RAS$_{7\text{B}}$ & RAS$_{\text{Sonnet-3.5}}$ &78.7  &54.7 &58.8  &70.8 &91.2 &39.1 &70.5  & 23.3 &37.7\\
RAS$_{8\text{B}}$  &73.8 & 44.2 &57.7 &77.6 & 71.4 &37.6 &96.2 &20.1 &54.4 \\
RAS$_{7\text{B}}$  &\textcolor{firstopen}{\underline{72.7}} &\textcolor{firstopen}{\underline{42.1}} &\textcolor{firstopen}{\underline{58.3}}  &\textcolor{secondopen}{\underline{74.7}} &\textcolor{firstopen}{\underline{68.5}} &\textcolor{firstopen}{37.2} &\textcolor{secondopen}{\underline{95.2}} & \textcolor{firstopen}{\underline{19.7}} &\textcolor{secondopen}{\underline{47.8}} \\
% [2pt]
% \hdashline[2pt/2pt] \\ [-9pt]
\bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{\small \textbf{Performance Comparison.} We highlight the \textcolor{firstclose}{top-2 closed-source models} and \textcolor{firstopen}{top-2 open-source 7B models}, underlining the \underline{best closed-/open-source (7B) model} for each dataset. Note: RAS is designed for general open-domain question answering and is not tailored for Knowledge Graph Question Answering (KGQA) tasks~\citep{perevalov-etal-2022-knowledge}; therefore, we do not compare it to KGQA-focused methods~\citep{sun2023think,luo2023reasoning,ma2024think}.}
\label{tb:main_results}
\vspace{-1em}
\end{table*}
